FiVA: Fine-grained Visual Attribute Dataset for Text-to-Image Diffusion Models

Recent advances in text-to-image generation have enabled the creation of high-quality images with diverse applications. However, accurately describing desired visual attributes can be challenging, especially for non-experts in art and photography. An intuitive solution involves adopting favorable attributes from the source images. Current methods attempt to distill identity and style from source images. However, "style" is a broad concept that includes texture, color, and artistic elements, but does not cover other important attributes such as lighting and dynamics. Additionally, a simplified "style" adaptation prevents combining multiple attributes from different sources into one generated image. In this work, we formulate a more effective approach to decompose the aesthetics of a picture into specific visual attributes, allowing users to apply characteristics such as lighting, texture, and dynamics from different images. To achieve this goal, we constructed the first fine-grained visual attributes dataset (FiVA) to the best of our knowledge. This FiVA dataset features a well-organized taxonomy for visual attributes and includes around 1 M high-quality generated images with visual attribute annotations. Leveraging this dataset, we propose a fine-grained visual attribute adaptation framework (FiVA-Adapter), which decouples and adapts visual attributes from one or more source images into a generated one. This approach enhances user-friendly customization, allowing users to selectively apply desired attributes to create images that meet their unique preferences and specific content requirements.

==> tables/clip_results.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \small
  \caption{\textbf{CLIP-score for subject accuracy measurement.} Our method shows the highest subject alignment on both in-domain and out-domain scenarios.}
    \begin{tabular}{c|l|ccccc}
    \toprule
    \multirow{3}[6]{*}{CLIP-Score} & Subject & \multicolumn{1}{l}{DB-Lora} & \multicolumn{1}{l}{IP-Adapter} & \multicolumn{1}{l}{DEADiff} & \multicolumn{1}{l}{StyleAligned} & \textbf{Ours} \\
\cmidrule{2-7}          & in-domain & 0.180 & 0.161 & 0.211 & 0.196 & \textbf{0.228} \\
\cmidrule{2-7}          & out-domain & 0.177 & 0.135 & 0.205 & 0.189 & \textbf{0.229} \\
    \bottomrule
    \end{tabular}%
  \label{tab:clip_score}%
\end{table}%


